ASASSN-18aan: An Eclipsing SU UMa-type Cataclysmic Variable with a 3.6-hour Orbital Period and a Late G-type Secondary Star

We report photometric and spectroscopic observations of the eclipsing SU UMa-type dwarf nova ASASSN-18aan. We observed the 2018 superoutburst with 2.3 mag brightening and found the orbital period ($P_{\rm orb}$) to be 0.149454(3) d, or 3.59 hr. This is longward of the period gap, establishing ASASSN-18aan as one of a small number of long-$P_{\rm orb}$ SU UMa-type dwarf novae. The estimated mass ratio, ($q=M_2/M_1 = 0.278(1)$), is almost identical to the upper limit of tidal instability by the 3:1 resonance. From eclipses, we found that the accretion disk at the onset of the superoutburst may reach the 3:1 resonance radius, suggesting that the superoutburst of ASASSN-18aan results from the tidal instability. Considering the case of long-$P_{\rm orb}$ WZ Sge-type dwarf novae, we suggest that the tidal dissipation at the tidal truncation radius is enough to induce SU UMa-like behavior in relatively high-$q$ systems such as SU UMa-type dwarf novae, but that this is no longer effective in low-$q$ systems such as WZ Sge-type dwarf novae. The unusual nature of the system extends to the secondary star, for which we find a spectral type of G9, much earlier than typical for the orbital period, and a secondary mass $M_2$ of around 0.18 M$_{\odot}$, smaller than expected for the orbital period and the secondary's spectral type. We also see indications of enhanced sodium abundance in the secondary's spectrum. Anomalously hot secondaries are seen in a modest number of other CVs and related objects. These systems evidently underwent significant nuclear evolution before the onset of mass transfer. In the case of ASASSN-18aan, this apparently resulted in a mass ratio lower than typically found at the system's $P_{\rm orb}$, which may account for the occurrence of a superoutburst at this relatively long period.

==> photjournal.tex <==
2019-09-05 07:38  &  -01:36 -- +02:41  &  30  &  510  &  GG420  \\
2019-09-06 07:11  &  -01:59 -- +02:15  &  60  &  249  &  R  \\
2019-09-08 06:15  &  -02:48 -- +01:40  &  30  &  357  &  GG420  \\
2019-10-22 03:37  &  -02:30 -- +02:43  &  30  &  553  &  GG420  \\
2019-10-23 07:18  &  +01:16 -- +03:42  &  30  &  274  &  GG420  \\
2019-10-24 03:03  &  -02:56 -- +02:11  &  33  &  475  &  GG420  \\

